Using Program Knowledge Graph to Uncover Software Vulnerabilities

In an increasingly interconnected and data-driven world, the importance of robust security measures cannot be overstated. A knowledge graph constructed with information extracted from the system along with the desired security behavior can be utilized to identify complex security vulnerabilities hidden underneath the systems. Unfortunately, existing security knowledge graphs are constructed from coarse-grained information extracted from publicly available vulnerability reports, which are not equipped to check actual security violations in real-world system implementations. In this poster, we present a novel approach of using Program Knowledge Graph that is embedded with fine-grained execution information of the systems (e.g., callgraph, data-flow, etc.) along with information extracted from the public vulnerability and weakness datasets (e.g., CVE and CWE). We further demonstrate that our custom security knowledge graph can be checked against the standard queries generated by LLM, providing a powerful way to identify security vulnerabilities and weaknesses in critical systems.

==> 02-background.tex <==
\section{Background}
\subsection{What are call graphs}
Call graphs represent the calling relationships among subroutines in computer programs, elucidating how functions or methods interact during program execution. Nodes in a call graph are functions or methods, and edges \textit{(f, g)} represents that procedure \textit{f} calls procedure \textit{g}.
\subsection{What are knowledge graphs}
The graph structure of knowledge graphs is \textit{G=(V, E, P)}. \textit{V} is a set of all nodes. \textit{E} is a set of all edges connecting nodes to represent relationships between entities.  \textit{P} is a set of triplet forms \textit{<concept, attribute, value>} associated with nodes or edges to provide additional information about the entities or relationships.
\subsection{Why Neo4j}
Leading graph databases such as Neo4j, OrientDB, and OntoText GraphDB offer powerful platforms for these representations. In this poster, we leverage Neo4j, a popular open-source graph database written in Java, as our database backend. The Neo4j databases can take in CSV format input files to construct knowledge graphs, and Neo4j’s built-in Cypher query language simplifies complex graph relationship expressions and traversal logic. In addition to Cypher, Neo4j provides support for Gremlin, a graph traversal and query language. Users can write their own graph traversal algorithms utilizing Gremlin and execute those algorithms via Neo4j’s REST API. Furthermore, Neo4j integrates with LLMs such as LangChain, Vertex AI, and OpenAI.



==> 04-analysis.tex <==
\section{Analysis}
In Neo4j, constructing a knowledge graph necessitates the initial development of a data model. Figure 1 portrays the data model for the knowledge graph. The CVE node represents Common Vulnerabilities and Exposures (CVE) entities, containing relevant properties. The CWE node denotes Common Weakness Enumeration (CWE) entities and stores associated properties. In the model, we also store the impact (CVSS2 score) of the CVE and affected product versions. The AFFECTS relationship indicates the CVE affects the product versions, the HAS\_CVE relationship indicates the CVE is an instance of the CWE type, and the SCORED relationship indicates the CVE has the CVSS2 scores. For CWE nodes, we store properties:
\begin{itemize}
    \item \texttt{CWE-ID}: A unique identifier of the CWE weakness.
    \item \texttt{Name}: Name of the CWE weakness.
    \item \texttt{Description}: An explanation of the CWE weakness.
    \item \texttt{Function Events}: Procedures that could potentially cause the corresponding weaknesses.
\end{itemize}
\includegraphics[width=\columnwidth]{figure/KGmodel.png}
\begin{center}
Figure 1. Data Model of the Knowledge Graph  
\end{center}

The process for constructing a call graph within Neo4j mirrors that of a knowledge graph. Figure 2 illustrates the model for the call graph. The CallGraph node represents the functions or methods, and the directed relationship CALLS indicates the caller Callgraph node calls the callee Callgraph node. As an example, Table 1 showcases node properties for the call graph in the context of the code snippet in Figure 3. The ExecOrder property is the sequence of procedure execution. The function gets with an ExecOrder 3 is executed prior to the function malloc with an ExecuOrder of 4. The Name property is the functions' or methods' names, while the property Argument1 stores the arguments passed in. It's important to note that users retain the flexibility to introduce additional \textit{Argument} properties as required to accommodate varying needs. 
%Figure 4 shows the call graph derived from the aforementioned code snippet, as stored within the Neo4j database.
%\begin{center}
%    \includegraphics[width=0.5\columnwidth]{figure/CallGraphmodel.png}
    
%    Figure 2. Data Model of the Call Graph
%\end{center}
%\begin{center}
\begin{tabular}{|c|c|c|} 
 \hline
 ExecOrder & Name & Argument1 \\
 1 & foo &  \\ 
 2 & printf & Please enter your name:\textbackslash n \\ 
 3 & gets & buf \\ 
 4 & malloc & 8 \\
 5 & doSomething & ptr \\
 6 & free & ptr \\
 7 & free & ptr \\
 \hline
\end{tabular}
Table 1. Node Properties of the Call Graph
\end{center}
\begin{lstlisting}
void foo()
{
    char buf[24];
    printf("Please enter your name:\n");
    gets(buf);
    char* ptr = (char*)malloc(8);
    doSomething(ptr);
    free(ptr);
    free(ptr);
}
\end{lstlisting}
\centerline{Figure 3. Example C Code}
%\begin{center}
%    \includegraphics[width=\textwidth]{figure/callgraphexample.png}
    
%    Figure 4. Call Graph with Procedure Names and Arguments Displayed on Each Node
%\end{center}



==> 05-experiments.tex <==
\section{Experiments and Evaluation}
The research aims to formulate Cypher queries using the information stored in the graph database to identify vulnerabilities in software code. Table 2 lists the comprehensive set of CWEs solely involving procedure calls for C/C++ software programs. 
%\begin{center}
%\begin{tabular}
%{|p{0.2\columnwidth}|p{0.45\columnwidth}|p{0.2\columnwidth}|}
%\hline
%    CWE-ID & Name & Function Events \\
    % \hline
%    CWE-134 & Use of Externally-Controlled Format String & printf, snprintf \\
    % \hline
%    CWE-242 & Use of Inherently Dangerous Function & gets, atoi, atol, atof \\
    % \hline
 %   CWE-243 & Creation of chroot Jail Without Changing Working Directory & chdir \\
    % \hline
%    CWE-244 & Improper Clearing of Heap Memory Before Release & realloc \\
    % \hline
%    CWE-401 & Missing Release of Memory after Effective Lifetime & free \\
    % \hline
%    CWE-415 & Double Free & free \\
    % \hline
%    CWE-467 & Use of sizeof() on a Pointer Type & sizeof \\
    % \hline
%    CWE-477 & Use of Obsolete Function & getpw, auto_ptr \\
    % \hline
%    CWE-479 & Signal Handler Use of a Non-reentrant Function & syslog \\
    % \hline
%    CWE-558 & Use of getlogin() in Multithreaded Application & getlogin \\
    % \hline
%    CWE-676 & Use of Potentially Dangerous Function & strcpy \\
    % \hline
%    CWE-1341 & Multiple Releases of Same Resource or Handle & fclose, free \\
%\hline
%\end{tabular}
%Table 2. Detectable CWEs Using Call Graphs and Knowledge Graphs
%\end{center}

In this section, we are going to present how to come up with Cypher queries to check if the program code shown in Figure 4 contains CWE weaknesses such as %CWE-242 (Use of Inherently Dangerous Function)\cite{CWE-242} and 
CWE-415 (Double Free)\cite{CWE-415}.

%\textbf{CWE-242}.  For CWE-242, we need to identify instances where the code calls a procedure that exhibits inherently dangerous behavior. For instance, the gets function copies input from STDIN to its argument without verifying the input size, which could potentially result in an overflow condition. To detect the presence of CWE-242 in the code, we execute the Cypher query shown in Figure 4. The first MATCH clause matches a node labeled as CWE where the value of the property CWE-ID is CWE-242. All nodes labeled as CallGraph are assigned an alias callgraph where the value of the property Name matches any of the values of Function Events property stored in the cwe node (from the previous match). OPTIONAL MATCH returns NULL when there are no CallGraph nodes that meet the condition. The second MATCH clause finds a shortest path starting from the entry point of the call graph, foo, to previously matched callgraph node (i.e., the node representing a function related to CWE-242). The WHERE clause filters the matched paths. It ensures that only paths with a length greater than 0 are considered. The RETURN clause returns the matched paths. In this query, the specification of dangerous function or method calls for assessment is unnecessary since the CWE-242 node already holds the Function Events property that keeps procedure examples that underlie the vulnerabilities associated with CWE-242. Figure 5 shows the result of the query. We can see the vulnerable path is returned, and the query successfully detects the CWE-242 in the code snippet.
%\begin{lstlisting}[language=Cypher]
%MATCH (cwe:CWE {`CWE-ID`: "CWE-242"})
%OPTIONAL MATCH (callgraph:CallGraph {Name: cwe.`Function Events`})
%MATCH path=shortestpath((CallGraph {Name: "foo"})-[*]->(callgraph))
%WHERE length(path) > 0
%RETURN path
%\end{lstlisting}
%\centerline{Figure 4. Sample Cypher Query to Detect CWE-242}
%\begin{center}
%    \includegraphics[width=\columnwidth]{figure/CWE-242-result.png}
    
%    Figure 5. Vulnerable Path Associated with CWE-242
%\end{center}

\textbf{CWE-415}. For CWE-415, a program calls free twice on the same memory address. This is an undefined behavior, potentially corrupting the program’s memory management data structures. To ascertain the potential presence of CWE-415 as an inherent vulnerability, the Cypher query depicted in Figure 6 is executed. We harness the properties stored within the CWE-415 node to check against the code snippet shown in Figure 4. The formulated query locates all nodes labeled as CallGraph with procedure names identical to the values stored within the Function Events property of the cwe node. Upon identification, these nodes are categorized based on their Argument1 property. Subsequently, the query examines whether the frequency of the procedure (such as free) being invoked on the same argument is greater than one. In cases where this condition is met, the query returns paths indicative of the vulnerability. It is worth noting that, in addition to the graphical representation, Neo4j furnishes a tabular representation - as exemplified in Table 3 - portraying the returned paths. Notably, both returned paths culminate in a function named free with an identical argument. This approach effectively detects the vulnerable code associated with CWE-415 within the code excerpt presented in Figure 4.
\begin{lstlisting}[language=Cypher]
MATCH (cwe:CWE {`CWE-ID`: "CWE-415"})
OPTIONAL MATCH (callgraph:CallGraph {Name: cwe.`Function Events`})
WITH callgraph.Argument1 AS argument1, COLLECT(callgraph) AS sameArgument1
WITH argument1, sameArgument1, SIZE(sameArgument1) AS nodeCount
WHERE nodeCount > 1
UNWIND sameArgument1 AS buggyNodes
OPTIONAL MATCH path=(startingNode:CallGraph {Name: "foo"})-[*]->(buggyNodes)
RETURN path
\end{lstlisting}
\centerline{Figure 6. Sample Cypher Query to Detect CWE-415}
\begin{center}
\begin{tabular}{|p{0.15\columnwidth}|p{0.7\columnwidth}|}
\hline
    Path 1 & (:CallGraph {ExecOrder: 1, Name: "foo"})-[:CALLS]->(:CallGraph {Argument1: "ptr", ExecOrder: 6, Name: "free"}) \\
    Path 2 & (:CallGraph {ExecOrder: 1, Name: "foo"})-[:CALLS]->(:CallGraph {Argument1: "ptr", ExecOrder: 7, Name: "free"}) \\
\hline
\end{tabular}
Table 3. Vulnerable Paths with Terminal Procedures \textit{free} Called on the Same Argument
\end{center}

